Lepton polarization asymmetries for FCNC decays of the $\Lambda_b$ baryon

Branching ratios, lepton forward-backward asymmetries, and lepton polarization asymmetries for the flavor-changing neutral current (FCNC) dileptonic decays of the $\Lambda_b$ baryon to the ground state and a number of excited state $\Lambda$ baryons are calculated using form factors extracted using wave functions from a constituent quark model. The SM branching ratios for the transition to the ground state calculated using these quark model form factors are consistent with the recent measurement reported by the LHCb collaboration. It is shown that the lepton polarization asymmetries are largely insensitive to the transition form factors and, therefore, to the effects of QCD in the nonperturbative regime. These observables can therefore provide somewhat model independent ways of extracting various combinations of the Wilson coefficients.

==> hqet.tex <==
\section{Heavy Quark Effective Theory\label{sec:hqet}}

Heavy quark effective theory (HQET) is an effective tool for examining the phenomenology of hadrons containing a single heavy quark. It has been
applied to hadronic matrix elements in many processes at higher and higher order in the $1/m_Q$ expansion, with $m_Q$ being the mass of the heavy
quark. In this section we present the leading-order relationships among the HQET form factors and those presented in Section \ref{sec:bme} for the
heavy to light transitions $\Lambda_b\rightarrow\Lambda^{(*)}$. The properties of the spinor-tensors that are used to represent the daughter baryons
have been discussed near the start of section \ref{sec:bme}.

To leading order in HQET, transitions between a heavy baryon and a light one are described in terms of only two form factors. For any current operator
$\Gamma$, the hadronic matrix elements involving tensor states can be written as \cite{mrr}
\begin{equation}
 \langle \Lambda^{(*)}(p_{\Lambda^{(*)}})\mid \overline{s}\Gamma b\mid
\Lambda_{b}(v)\rangle=\overline{u}_{\mu_1\ldots\mu_n}(p_{\Lambda^{(*)}})M^{\mu_1\ldots\mu_n}\Gamma
u(v) \label{eq:hqetme}
\end{equation}
where $v$ is the velocity of the $\Lb$ baryon and $M^{\mu_1\ldots\mu_n}$ is the most general tensor consistent with HQET that can be constructed from
the available kinematic variables. We may not use any factors of $\gamma^{\mu_i}$, $p_{\Lambda^{(*)}}^{\mu_i}$, or $g^{\mu_i\mu_j}$ in constructing
$M^{\mu_1\ldots\mu_n}$; therefore, it must take the form
\begin{equation}
M^{\mu_1\ldots\mu_n}=v^{\mu_1}\ldots v^{\mu_n}\bigg[\xi^{(n)}_{1}(v\cdot p_{\Lambda^{(*)}})+\slash{v}\xi^{(n)}_{2}(v\cdot p_{\Lambda^{(*)}})\bigg],
\end{equation}
For the case of a pseudo-tensor daughter baryon, the matrix element has the same form as Eq. \ref{eq:hqetme} except that $M^{\mu_1\ldots\mu_n}$ is now
a pseudo-tensor. A pseudo-tensor when sandwiched between spinors can be constructed by multiplying an ordinary tensor by $\gamma_5$; thus, for
transitions involving a pseudo-tensor spinor,
\begin{equation}
M^{\mu_1\ldots\mu_n}=v^{\mu_1}\ldots v^{\mu_n}\bigg[\zeta^{(n)}_{1}(v\cdot p_{\Lambda^{(*)}})+\slash{v}\zeta^{(n)}_{2}(v\cdot
p_{\Lambda^{(*)}})\bigg]\gamma_5.
\end{equation}
Using these forms of the matrix elements, the form factors defined in Section \ref{sec:bme} are found to satisfy the following  relations in the limit
when the $b$ quark is infinitely heavy.

For any state with $J^P=1/2^{+}$,
\begin{eqnarray}
F_3&=&G_3=H_3=H_4=0, \,\,\,\, F_2=G_2=-H_2=2\xi^{(0)}_2, \nonumber \\ F_1&=&\xi^{(0)}_1-\xi^{(0)}_2, \,\,\,\, G_1=H_1=\xi^{(0)}_1+\xi^{(0)}_2,
\label{eq:hqet12p}
\end{eqnarray}
while for $J^P=1/2^{-}$, we have
\begin{eqnarray}
F_3&=&G_3=H_3=H_4=0, \,\,\,\, F_2=G_2=H_2=-2\zeta^{(0)}_2, \nonumber \\ F_1&=&-\left[\zeta^{(0)}_1+\zeta^{(0)}_2\right], \,\,\,\,
G_1=-H_1=-\left[\zeta^{(0)}_1-\zeta^{(0)}_2\right].
\label{eq:hqet12m}
\end{eqnarray}
For $J^P=3/2^{-}$,
\begin{eqnarray}
F_3&=&G_3=H_3=F_4=G_4=H_4=H_5=H_6=0, \,\,\,\, F_2=G_2=-H_2=2\xi^{(1)}_2, \nonumber \\ F_1&=&\xi^{(1)}_1-\xi^{(1)}_2, \,\,\,\,
G_1=H_1=\xi^{(1)}_1+\xi^{(1)}_2.
\label{eq:hqet32m}
\end{eqnarray}
For $J^P=3/2^{+}$,
\begin{eqnarray}
F_3&=&G_3=H_3=F_4=G_4=H_4=H_5=H_6=0, \,\,\,\, F_2=G_2=H_2=-2\zeta^{(1)}_2, \nonumber \\ F_1&=&-\left[\zeta^{(1)}_1+\zeta^{(1)}_2\right], \,\,\,\,
G_1=-H_1=-\left[\zeta^{(1)}_1-\zeta^{(1)}_2\right].
\label{eq:hqet32p}
\end{eqnarray}
For $J^P=5/2^{+}$,
\begin{eqnarray}
F_3&=&G_3=H_3=F_4=G_4=H_4=H_5=H_6=0, \,\,\,\, F_2=G_2=-H_2=2\xi^{(2)}_2, \nonumber \\ F_1&=&\xi^{(2)}_1-\xi^{(2)}_2, \,\,\,\,
G_1=H_1=\xi^{(2)}_1+\xi^{(2)}_2.
\label{eq:hqet52p}
\end{eqnarray}
Again, we stress that the above relationships are for heavy to light transitions only, and are valid in the limit of an infinitely heavy $b$ quark.


==> pol_results.tex <==
\section{Results\label{sec:results}}

\subsection{Form Factors and Branching Ratios}

For the numerical calculations, we use form factors that result from the SCA and MCN approaches outlined in \cite{morob}. The parameters for the quark model wave functions used in the extraction of the form factors are taken from \cite{roper} and are given in Tables \ref{hampar} and \ref{qmtab}. The form factors calculated using the SCA model have the form
\beq
F(\sh)=A_0\exp\left(-\frac{3m_q^2}{2\tilde m_\Lambda^2}\frac{p_\Lambda^2}{\alpha_{\lambda\lambda'}^2}\right),
\label{eq:scaff}
\eeq
where $A_0$ is the value of the form factor at the nonrecoil point, $m_q$ is the mass of each light quark,
$\alpha_{\lambda\lambda'}=\sqrt{(\alpha_{\lambda}^{2}+\alpha_{\lambda'}^{2})/2}$, $\tilde{m}_\Lambda=m_s+2m_q$, and $\pls=\mlb\sqrt{\phi(\sh)}/2$ is the daughter baryon momentum in the $\Lb$ rest frame. The explicit expressions for these form factors are given in Appendix \ref{sec:aff}. The form factors calculated using the MCN model are parametrized to have the form
\beq
F(\sh)=(a_0+a_2\pls^2+a_4\pls^4)\exp\left(-\frac{3m_q^2}{2\tilde m_\Lambda^2}\frac{p_\Lambda^2}{\alpha_{\lambda\lambda'}^2}\right).
\label{eq:mcnff}
\eeq
The parameters $a_0$, $a_2$, and $a_4$ for the vector and axial vector form factors are given in Table \ref{vaff}. The parameters for the tensor form factors are given in Table \ref{tff}.

\begin{table}
\caption{Hamiltonian parameters obtained from a fit to a selection of known baryons.}
\label{hampar}
\begin{tabular}{cccccccccc}
\hline\small $m_q$ &\small $m_s$ &\small $m_c$ &\small $m_b$ &\small $b$ &\small $\alf_{coul}$ &\small $\alf_{con}$ &\small $\alf_{SO}$ &\small $\alf_{tens}$ &\small $C_{qqq}$ \\
\small (${\text{GeV}}$) &\small (${\text{GeV}}$) &\small (${\text{GeV}}$) &\small (${\text{GeV}}$) &\small (${\text{GeV}^2}$) & & &\small (${\text{GeV}}$) & &\small ($\text{GeV}$) \\ \hline
\small $0.2848$ &\small $0.5553$ &\small $1.8182$ &\small $5.2019$ &\small $0.1540$ &\small $\approx0.0$ &\small $1.0844$ &\small $0.9321$ &\small $-0.2230$ &\small $-1.4204$ \\ \hline
\end{tabular}
\end{table}


\begin{table}
\caption{Baryon masses and wave function size parameters, $\alf_\rho$ and $\alf_\lambda$, for states with different $\jp$. All values are in GeV.}
\label{qmtab}
\begin{tabular}{ccccc}
\hline\small State, $J^{P}$ &\small Experiment &\small Model &\small $\alf_\lambda$  &\small $\alf_\rho$ \\ \hline
\small$\Lambda_b(5620)\,1/2^{+}$ &\small $5.62$ &\small $5.61$ &\small $0.443$ &\small $0.385$  \\ \hline
\small$\Lambda(1115)\,1/2^{+}$   &\small $1.12$ &\small $1.10$ &\small $0.387$ &\small $0.372$  \\ \hline
\small$\Lambda(1600)\,1/2^{+}$   &\small $1.60$ &\small $1.71$ &\small $0.387$ &\small $0.372$  \\ \hline
\small$\Lambda(1405)\,1/2^{-}$   &\small$1.41$  &\small $1.48$ &\small $0.333$ &\small $0.320$  \\ \hline
\small$\Lambda(1520)\,3/2^{-}$   &\small $1.52$ &\small $1.53$ &\small $0.333$ &\small $0.308$  \\ \hline
\small$\Lambda(1890)\,3/2^{+}$   &\small $1.89$ &\small $1.81$ &\small $0.325$ &\small $0.303$  \\ \hline
\small$\Lambda(1820)\,5/2^{+}$   &\small $1.82$ &\small $1.81$ &\small $0.325$ &\small $0.303$  \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Coefficients in the parametrization of the vector and axial-vector form factors obtained in the MCN approach.}\label{vaff}
\begin{tabular}{cccccccccc}
\hline                      & $a_n(\text{GeV}^{-n})$ & $F_1$ & $F_2$ & $F_3$ & $F_4$ & $G_1$ & $G_2$ & $G_3$ & $G_4$ \\ \hline
                            &  $a_0$ & $1.14$       & $-0.137$     & $-0.0614$    & $-$ & $0.923$     & $-0.171$    & $0.0779$    & $-$ \\
$\Lambda_b\to\Lambda(1115)$ &  $a_2$ & $0.0434$     & $-0.00408$   & $0.00249$    & $-$ & $0.0466$    & $0.000477$  & $-0.00162$  & $-$ \\
                            &  $a_4$ & $-0.000879$  & $0.00164$    & $-0.00113$   & $-$ & $-0.000293$ & $0.00121$   & $0.000386$  & $-$ \\ \hline
                            &  $a_0$ & $0.420$      & $-0.328$     & $0.0470$     & $-$ & $0.116$     & $-0.352$    & $-0.0304$   & $-$ \\
$\Lambda_b\to\Lambda(1600)$ &  $a_2$ & $0.433$      & $-0.122$     & $-0.0297$    & $-$ & $0.286$     & $-0.140$    & $0.0424$    & $-$ \\
                            &  $a_4$ & $0.0102$     & $0.00362$    & $-0.000788$  & $-$ & $0.0139$    & $-0.00434$  & $0.000227$  & $-$ \\ \hline
                            &  $a_0$ & $0.245$      & $-0.907$     & $0.112$      & $-$ & $1.09$      & $-0.806$    & $0.00493$   & $-$ \\
$\Lambda_b\to\Lambda(1405)$ &  $a_2$ & $0.130$      & $-0.0980$    & $0.0178$     & $-$ & $0.212$     & $-0.0901$   & $-0.0141$   & $-$ \\
                            &  $a_4$ & $0.00123$    & $0.00674$    & $-0.000442$  & $-$ & $-0.00439$  & $0.00610$   & $0.000269$  & $-$ \\ \hline
                            &  $a_0$ & $-1.30$      & $0.259$      & $0.120$      & $-0.0323$    & $-0.907$     & $0.310$      & $-0.153$     &
$0.0532$ \\
$\Lambda_b\to\Lambda(1520)$ &  $a_2$ & $-0.0828$    & $0.0149$     & $0.00232$    & $-0.00895$   & $-0.0747$    & $0.0130$     & $-0.00269$   &
$-0.00154$ \\
                            &  $a_4$ & $0.00500$    & $-0.00308$   & $0.000161$   & $0.00225$    & $0.00278$    & $-0.00313$   & $0.000130$   &
$-0.000350$ \\ \hline
                            &  $a_0$ & $-0.369$     & $1.31$       & $-0.218$     & $0.0457$     & $-1.60$      & $1.13$       & $0.0212$     &
$-0.0142$ \\
$\Lambda_b\to\Lambda(1890)$ &  $a_2$ & $-0.150$     & $0.0819$     & $-0.0235$    & $0.0128$     & $-0.222$     & $0.0761$     & $0.0195$     &
$-0.00540$ \\
                            &  $a_4$ & $-0.000684$  & $0.000189$   & $-0.0000847$ & $-0.00217$   & $-0.000644$  & $-0.000109$  & $-0.000261$  &
$0.000566$ \\ \hline
                            &  $a_0$ & $1.84$       & $-0.426$     & $-0.190$     & $0.0768$     & $1.18$       & $-0.520$       & $0.270$      &
$-0.114$ \\
$\Lambda_b\to\Lambda(1820)$ &  $a_2$ & $0.0899$     & $-0.00558$   & $-0.00640$   & $0.00385$    & $0.0909$     & $-0.00116$     & $0.00270$     &
$-0.00259$ \\
                            &  $a_4$ & $-0.000260$  & $0.000242$   & $-0.000159$  & $-0.0000581$ & $-0.000923$  & $-0.000167$    & $0.000501$   &
$0.0000289$ \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Coefficients in the parametrization of the tensor form factors obtained in the MCN approach.}\label{tff}
\begin{tabular}{cccccccc}
\hline                      & $a_n(\text{GeV}^{-n})$ & $H_1$ & $H_2$ & $H_3$ & $H_4$ & $H_5$ & $H_6$ \\ \hline
                            &  $a_0$ & $0.930$      & $0.165$      & $-0.0771$    & $-0.0135$    & $-$ & $-$ \\
$\Lambda_b\to\Lambda(1115)$ &  $a_2$ & $0.0193$     & $0.0269$     & $-0.000141$  & $-0.00309$   & $-$ & $-$ \\
                            &  $a_4$ & $-0.00123$   & $-0.00274$   & $0.0000809$  & $0.00110$    & $-$ & $-$ \\ \hline
                            &  $a_0$ & $0.124$      & $0.346$      & $0.0294$     & $-0.00441$   & $-$ & $-$ \\
$\Lambda_b\to\Lambda(1600)$ &  $a_2$ & $0.290$      & $0.136$      & $-0.0425$    & $-0.0191$    & $-$ & $-$ \\
                            &  $a_4$ & $0.00846$    & $0.00109$    & $-0.000222$  & $0.00102$    & $-$ & $-$ \\ \hline
                            &  $a_0$ & $-1.07$      & $-0.805$     & $0.00262$    & $-0.101$     & $-$ & $-$ \\
$\Lambda_b\to\Lambda(1405)$ &  $a_2$ & $-0.213$     & $-0.0920$    & $-0.0141$    & $-0.00522$   & $-$ & $-$ \\
                            &  $a_4$ & $0.00457$    & $0.00629$    & $0.000257$   & $0.000386$   & $-$ & $-$ \\ \hline
                            &  $a_0$ & $-1.02$      & $-0.200$     & $0.153$      & $0.0516$     & $-0.0524$    & $0.0156$ \\
$\Lambda_b\to\Lambda(1520)$ &  $a_2$ & $-0.0360$    & $-0.0516$    & $0.00271$    & $-0.00354$   & $0.00158$    & $0.00218$ \\
                            &  $a_4$ & $0.000522$   & $0.00538$    & $-0.000132$  & $0.000186$   & $-0.000349$  & $-0.00109$ \\ \hline
                            &  $a_0$ & $1.57$       & $1.12$       & $0.0233$     & $0.186$      & $-0.0136$    & $0.0316$ \\
$\Lambda_b\to\Lambda(1890)$ &  $a_2$ & $0.222$      & $0.0768$     & $0.0197$     & $0.00454$    & $-0.00587$   & $0.00775$  \\
                            &  $a_4$ & $0.000636$   & $-0.000109$  & $-0.000271$  & $0.000307$   & $0.000576$   & $-0.00166$ \\ \hline
                            &  $a_0$ & $1.41$       & $0.286$      & $-0.270$     & $-0.0855$    & $0.114$      & $-0.0365$ \\
$\Lambda_b\to\Lambda(1820)$ &  $a_2$ & $0.0484$     & $0.0436$     & $-0.00270$   & $0.00432$    & $0.00261$    & $0.00114$ \\
                            &  $a_4$ & $0.000542$   & $-0.00130$   & $-0.000501$  & $-0.000387$  & $-0.0000296$ & $-0.00000613$ \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{}\label{hqetff}
\begin{tabular}{cccc}
\hline                      & $\xiv_2/\xiv_1$ & $\xia_2/\xia_1$ & $\xit_2/\xit_1$  \\
                            & \small SCA $\,\,\,\,$ \small MCN & \small SCA $\,\,\,\,$ \small MCN & \small SCA $\,\,\,\,$ \small MCN \\ \hline
$\Lambda_b\to\Lambda(1115)$ & $-0.166\,\,\,\,\,\,-0.064$ & $-0.193\,\,\,\,\,\,-0.085$ & $-0.188\,\,\,\,\,\,-0.081$ \\ \hline
$\Lambda_b\to\Lambda(1600)$ & $-0.615\,\,\,\,\,\,-0.641$ & $-0.611\,\,\,\,\,\,-0.603$ & $-0.590\,\,\,\,\,\,-0.582$  \\ \hline
$\Lambda_b\to\Lambda(1405)$ & $-0.555\,\,\,\,\,\,-0.623$ & $-0.499\,\,\,\,\,\,-0.587$ & $-0.517\,\,\,\,\,\,-0.603$  \\ \hline
$\Lambda_b\to\Lambda(1520)$ & $-0.139\,\,\,\,\,\,-0.111$ & $-0.172\,\,\,\,\,\,-0.146$ & $-0.111\,\,\,\,\,\,-0.089$  \\ \hline
$\Lambda_b\to\Lambda(1890)$ & $-0.353\,\,\,\,\,\,-0.640$ & $-0.285\,\,\,\,\,\,-0.546$ & $-0.293\,\,\,\,\,\,-0.554$  \\ \hline
$\Lambda_b\to\Lambda(1820)$ & $-0.130\,\,\,\,\,\,-0.131$ & $-0.172\,\,\,\,\,\,-0.181$ & $-0.056\,\,\,\,\,\,-0.092$  \\ \hline
\end{tabular}
\end{table}

The SCA form factors have all of their kinematic dependence in the form of a Gaussian in the momentum of the daughter baryon (Eq. \ref{eq:scaff}), calculated in the rest frame of the parent, whereas the MCN form factors have an additional polynomial dependence in the daughter baryon's momentum (Eq. \ref{eq:mcnff}). Depending on the relative sizes of $a_0$ and $a_2$ in Eq. \ref{eq:mcnff}, the SCA and MCN form factors can have quite different shapes \cite{morob}.

\begin{table}
\caption{SM and SUSY values for the Wilson coefficients. In the SUSY model we use, only $C_7$, $C_9$, and $C_{10}$ get modified from their SM values.}
\label{wilco}
\begin{tabular}{cccccccccc}
\hline &\small $C_1$ &\small $C_2$ &\small $C_3$ &\small $C_4$ &\small $C_5$ &\small $C_6$ &\small $C_7$ &\small $C_9$ &\small $C_{10}$ \\ \hline
\small SM &\small $-0.243$ &\small $1.105$ &\small $0.011$ &\small $-0.025$ &\small $0.007$ &\small $-0.031$ &\small $-0.312$ &\small $4.193$ &\small
$-4.578$ \\ \hline
\small SUSY & & & & & & &\small $0.376$ &\small $4.767$ &\small $-3.735$ \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Branching ratios for $\Lambda_b\rightarrow \Lambda^{(*)}\mu^{+}\mu^{-}$ in units of $10^{-6}$. The numbers in the column labeled SM1 are obtained using the SCA form factors with standard model Wilson Coefficients. The numbers in the column labeled SM2 are also obtained using SM Wilson coefficients, but the MCN form factors. The numbers in the column labeled SUSY are obtained using the MCN form factors with Wilson coefficients from a supersymmetric scenario. The column labeled LD refers to the long distance contributions of the charmonium resonances, with `a' indicating that these contributions have been neglected, and `b' indicating that they have been included. In this table, it is assumed that the $\Lambda(1600)$ is the first radial excitation. The lifetime of the $\Lambda_b$ is taken from the Particle Data Listings \cite{pdg}.}
{\begin{tabular}{cccccccccc}
\hline\small State, $J^{P}$       & LD & SM1 &\small SM2 &\small SUSY &\small Aslam {\it et al.} \cite{aslam}  &\small Wang {\it et al.} \cite{wang} 
&\small Chen {\it et al.} \cite{chen} & CDF \cite{cdf2} & LHCb \cite{lhcb2} \\
&& & & && &\small QCDSR $\,\,$\small PM & \\ \hline
\small$\Lambda(1115)\,1/2^{+}$    & a &\small $0.66$  &\small $0.59$  &\small $0.86$  &\small $5.9$ &\small $6.1$ &\small $2.1$
$\,\,\,\,\,\,\,\,\,\,\,$ $1.2$ & $1.73\pm0.42\pm0.55$ & $0.96\pm0.16\pm0.13\pm0.21$ \\
                                  & b &\small $21$    &\small $20$    &\small $20$    &\small $39$  &\small $46$  &\small $53$
$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,$ $36$ & $-$ & $-$\\ \hline
\small$\Lambda(1600)\,1/2^{+}$    & a &\small $0.030$ &\small $0.23$  &\small $0.38$  & $-$ & $-$ & $-$& $-$ & $-$ \\
                                  & b &\small $2.6$   &\small $24$    &\small $24$    & $-$ & $-$ & $-$& $-$ & $-$ \\ \hline
\small$\Lambda(1405)\,1/2^{-}$    & a &\small $0.10$ &\small $0.15$  &\small $0.23$  & $-$ & $-$ & $-$& $-$ & $-$ \\
                                  & b &\small $5.9$   &\small $11$    &\small $11$    & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline
\small$\Lambda(1520)\,3/2^{-}$    & a &\small $0.14$  &\small $0.16$  &\small $0.25$  & $-$ & $-$ & $-$ & $-$ & $-$\\
                                  & b &\small $14$    &\small $16$    &\small $16$    & $-$ & $-$ & $-$& $-$ & $-$ \\ \hline
\small$\Lambda(1890)\,3/2^{+}$    & a &\small $0.018$ &\small $0.052$ &\small $0.088$ & $-$ & $-$ & $-$ & $-$ & $-$\\
                                  & b &\small $1.3$   &\small $3.3$   &\small $3.4$   & $-$ & $-$ & $-$& $-$ & $-$ \\ \hline
\small$\Lambda(1820)\,5/2^{+}$    & a &\small $0.013$ &\small $0.051$ &\small $0.090$ & $-$ & $-$ & $-$ & $-$ & $-$\\
                                  & b &\small $0.84$  &\small $3.1$   &\small $3.1$   & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline
\end{tabular}\label{br1}}
\end{table}

\begin{table}[H]
\caption{Branching ratios for $\Lambda_b\rightarrow \Lambda^{(*)}\tau^{+}\tau^{-}$ in units of $10^{-6}$. The columns are labeled as in Table
\ref{br1}.}
{\begin{tabular}{cccccccc}
\hline\small State, $J^{P}$     & LD &\small SM1 &\small SM2 &\small SUSY &\small Aslam {\it et al.} \cite{aslam}  &\small Wang {\it et al.}
\cite{wang}  &\small Chen {\it et al.} \cite{chen}  \\
&& & & && &\small QCDSR $\,\,$\small PM \\ \hline
\small$\Lambda(1115)\,1/2^{+}$  & a &\small $0.24$  &\small $0.21$  &\small $0.36$  &\small $2.1$ &\small $2.4$ &\small $0.18$
$\,\,\,\,\,\,\,\,\,\,\,$ $0.26$ \\
                                & b &\small $0.59$  &\small $0.52$  &\small $0.67$  &\small $4.0$ &\small $4.3$ &\small $11$
$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,$ $9.0$ \\ \hline
\small$\Lambda(1600)\,1/2^{+}$  & a &\small $<0.01$ &\small $<0.01$ &\small $0.015$ & $-$ & $-$ & $-$ \\
                                & b &\small $0.033$ &\small $0.096$ &\small $0.10$  & $-$ & $-$ & $-$ \\ \hline
\small$\Lambda(1405)\,1/2^{-}$  & a &\small $0.026$ &\small $0.025$ &\small $0.046$ & $-$ & $-$ & $-$ \\
                                & b &\small $0.12$  &\small $0.15$  &\small $0.17$  & $-$ & $-$ & $-$ \\ \hline
\small$\Lambda(1520)\,3/2^{-}$  & a &\small $0.015$ &\small $0.014$ &\small $0.028$ & $-$ & $-$ & $-$ \\
                                & b &\small $0.14$  &\small $0.14$  &\small $0.15$  & $-$ & $-$ & $-$ \\ \hline
\small$\Lambda(1890)\,3/2^{+}$  & a &\small $<0.01$ &\small $<0.01$ &\small $<0.01$ & $-$ & $-$ & $-$ \\
                                & b &\small $<0.01$ &\small $<0.01$ &\small $<0.01$ & $-$ & $-$ & $-$ \\ \hline
\small$\Lambda(1820)\,5/2^{+}$  & a &\small $<0.01$ &\small $<0.01$ &\small $<0.01$ & $-$ & $-$ & $-$ \\
                                & b &\small $<0.01$ &\small $<0.01$ &\small $<0.01$ & $-$ & $-$ & $-$ \\ \hline
\end{tabular}\label{br2}}
\end{table}

\subsection{Lepton Polarization Asymmetries}

In this section, we present SLPAs for dileptonic decays. We present SM results and results obtained from a SUSY extension of the SM. In our 
numerical calculations, the SM values of the Wilson coefficients are taken from \cite{huang} and the SUSY values are take from \cite{aslam} and are presented in Table \ref{wilco}. In \cite{huang} the Wilson coefficients were evaluated using a naive dimensional regularization scheme at the scale $\mu=5\text{ GeV}$. The top  quark mass was taken to be $m_t=174\text{ GeV}$ and the cut-off $\Lambda_{\overline{MS}}=225\text{ MeV}$, where $\overline{MS}$ denotes the modified minimal subtraction scheme. The SUSY model used here is referred to as SUSYI in Ref. \cite{aslam}. SUSYI corresponds to the regions of parameter space where supersymmetry can destructively contribute and can change the sign of $C_7$, but contributions from neutral Higgs bosons are neglected.

\subsubsection{Longitudinal Lepton Polarization Asymmetries}

\begin{table}
\caption{Integrated longitudinal lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\mu^{+}\mu^{-}$ in units of $10^{-2}$. The
numbers in the column labeled SM1 are obtained using the SCA form factors with standard model Wilson Coefficients. The numbers in the column labeled SM2 are also obtained using SM Wilson coefficients, but the MCN form factors. The numbers in the column labeled SUSY are obtained using the MCN form factors with Wilson coefficients from a supersymmetric scenario. The column labeled LD refers to the long distance contributions of the charmonium resonances, with `a' indicating that these contributions have been neglected, and `b' indicating that they have been included. In this table, it is assumed that the $\Lambda(1600)$ is the first radial excitation.}
{\begin{tabular}{cccccc}
\hline State, $J^{P}$       & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2} \\
& & & & &\small QCDSR $\,\,$\small PM  \\ \hline
$\Lambda(1115)\,1/2^{+}$    & a & $-58.1$ & $-58.5$ & $-53.2$ & $-58.3\,\,\,\,\,\,\,\,\,\,\,-58.3$ \\
                            & b & $-51.6$ & $-51.9$ & $-49.1$ &$-$ \\ \hline
$\Lambda(1600)\,1/2^{+}$    & a & $-45.4$ & $-45.6$ & $-41.4$ & $-$ \\
                            & b & $-40.1$ & $-40.4$ & $-37.1$ & $-$ \\ \hline
$\Lambda(1405)\,1/2^{-}$    & a & $-49.7$ & $-50.2$ & $-45.6$ & $-$ \\
                            & b & $-43.9$ & $-44.4$ & $-41.4$ & $-$ \\ \hline
$\Lambda(1520)\,3/2^{-}$    & a & $-46.7$ &  $-47.5$ & $-43.1$ & $-$ \\
                            & b & $-41.4$ & $-42.1$ & $-38.8$ & $-$ \\ \hline
$\Lambda(1890)\,3/2^{+}$    & a & $-38.1$ & $-38.3$ & $-34.8$ & $-$  \\
                            & b & $-34.1$ & $-34.2$ & $-30.3$ & $-$ \\ \hline
$\Lambda(1820)\,5/2^{+}$    & a & $-38.7$ & $-39.6$ & $-36.0$ & $-$  \\
                            & b & $-34.3$ & $-35.0$ & $-31.7$ & $-$ \\ \hline
\end{tabular}\label{llpa1}}
\end{table}

\begin{table}
\caption{Integrated longitudinal lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\tau^{+}\tau^{-}$ in units of $10^{-2}$. The columns are labeled as in Table \ref{llpa1}.}
{\begin{tabular}{ccccccc}
\hline State, $J^{P}$      & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2} \\
& & & & &\small QCDSR $\,\,$\small PM    \\ \hline
$\Lambda(1115)\,1/2^{+}$   & a & $-10.7$ & $-10.8$ & $-8.2$ & $-10.9\,\,\,\,\,\,\,\,\,\,\,-10.9$ \\
                           & b & $-10.2$ & $-10.3$ & $-8.1$ & $-$  \\ \hline
$\Lambda(1600)\,1/2^{+}$   & a & $-3.4$ & $-3.5$ & $-2.6$ & $-$ \\
                           & b & $-3.1$ & $-3.1$ & $-2.5$ & $-$  \\ \hline
$\Lambda(1405)\,1/2^{-}$   & a & $-5.9$ & $-6.0$ & $-4.5$ & $-$  \\
                           & b & $-5.5$ & $-5.6$ & $-4.4$ & $-$  \\ \hline
$\Lambda(1520)\,3/2^{-}$   & a & $-4.6$ &  $-4.6$ & $-3.4$ & $-$  \\
                           & b & $-4.2$ & $-4.2$ & $-3.2$ & $-$  \\ \hline
$\Lambda(1890)\,3/2^{+}$   & a & $-0.81$ & $-0.80$ & $-0.58$ & $-$  \\
                           & b & $-0.54$ & $-0.52$ & $-0.46$ & $-$  \\ \hline
$\Lambda(1820)\,5/2^{+}$   & a & $-1.4$ &  $-1.4$ & $-0.99$ & $-$  \\
                           & b & $-1.1$ & $-1.1$ & $-0.89$ & $-$  \\ \hline
\end{tabular}\label{llpa2}}
\end{table}

The integrated LLPAs we obtain are shown in Tables \ref{llpa1} and \ref{llpa2}. Each table displays the results for the SM calculations using two models for the form factors, as well as one SUSY scenario with the MCN form factors. In addition, results obtained omitting and including the long distance (LD) contributions are presented. We also compare our results for decays to the ground state with those of Chen {\it et al.} \cite{chen2}, where they have used QCD sum rules (QCDSR) and a pole model (PM) for the form factors. As can be seen, the results from both SM1a and SM2a are in agreement with each other and the QCDSR and PM results reported in \cite{chen2} for both channels. For decays to the excited states, the SM1 and SM2 results are in agreement for both channels as well. In the SUSY scenario we use, where $C_7^{SUSY}=-C_7^{SM}$, the LLPAs are quite different from the SM results for both channels.

\subsubsection*{$\it\jp=1/2^+$}


%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_12p_LO_inclusive_q2.eps}\,\,\,\,\,\,
\includegraphics[width=3.0in]{tau_slpa_L_12p_LO_inclusive_q2.eps}}
\caption{$\P_L^-(q^2)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$ without and with long distance (LD) contributions from charmonium resonances. The solid curves arise from the free quark process $b\to s\ell^+\ell^-$, while the dashed curves are the SM2 results, and the dot-dashed curves are the leading order SM results, $\D_L^{(0)-}/\D_0^{(0)}$.}\label{fig:PLq212p}
\end{figure}

In Fig. \ref{fig:PLq212p}, we show the differential LLPA as a functions of $q^2$ for decays to the ground state, $\Ls(1115)$ for the SM2 case. In addition, we also display results for the free-quark process $b\to s\ell^+\ell^-$ as well as the leading order HQET result with no form factor dependence, $\D_L^{(0)-}/\D_0^{(0)}$ (see Appendix \ref{sec:hqet}). It can be seen that these curves are nearly indistinguishable.

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_12p.eps}\,\,\,\,\,\,
\includegraphics[width=3.0in]{tau_slpa_L_12p.eps}}
\caption{$\P_L^-(\sh)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$ without and with long distance (LD) contributions from charmonium resonances. The solid and dashed curves represent SLPAs obtained from SCA and MCN form factors, respectively. The dash-dotted curves represent a SUSY extension to the SM.}\label{fig:PL12p}
\end{figure}

Fig. \ref{fig:PL12p} shows these same LLPAs as a function of $\sh$ for the SM1, SM2, and SUSY cases with and without LD contributions. The solid curves represent the results of SM1, the dashed curves are SM2 results, while SUSY results are the dot-dashed curves. The curves for the SM1 and SM2 cases are nearly indistinguishable over the entire kinematic range for the both the $\mu$ and $\tau$ channels. However, we see that there is a significant difference between the SM predictions and the  SUSY result in both channels. These observations are borne out by the results presented  in Tables \ref{llpa1} and \ref{llpa2}.

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_12p1r.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_L_12p1r.eps}}
\caption{Same as Fig. \ref{fig:PL12p} but for $\Lambda_{b}\rightarrow\Lambda(1600)$.}\label{fig:PL12p1r}
\end{figure}

Fig. \ref{fig:PL12p1r} shows the predictions for LLPAs for decays to $\Ls(1600)$ for SM1, SM2, and SUSY models with both LD scenarios. The SM1 and SM2 results are essentially identical for both channels and this is reflected in the values of the integrated LLPAs. Again, the SM and SUSY results are quite different.

\subsubsection*{$\it\jp=1/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_12m_00.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_L_12m_00.eps}}
\caption{Same as Fig. \ref{fig:PL12p} but for $\Lambda_{b}\rightarrow\Lambda(1405)$.}\label{fig:PL12m}
\end{figure}

The predictions for LLPAs for decays to $\Ls(1405)$ are shown in Fig. \ref{fig:PL12m}. As can be seen, the predictions from SM1 and SM2 are nearly identical in both channels. The SUSY prediction is quite different from the SM predictions in both channels.

\subsubsection*{$\it\jp=3/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_32m.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_L_32m.eps}}
\caption{Same as Fig. \ref{fig:PL12p} but for $\Lambda_{b}\rightarrow\Lambda(1520)$.}\label{fig:PL32m}
\end{figure}

In Fig. \ref{fig:PL32m}, the predictions for LLPAs for decays to $\Ls(1520)$ are shown. These figures show that the predictions from SM1 and SM2 are nearly identical while the SUSY prediction is quite different in both channels.

\subsubsection*{$\it\jp=3/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_32p_00.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_L_32p_00.eps}}
\caption{Same as Fig. \ref{fig:PL12p} but for $\Lambda_{b}\rightarrow\Lambda(1890)$.}\label{fig:PL32p}
\end{figure}

The predictions for LLPAs for decays to $\Ls(1890)$ are shown in Fig. \ref{fig:PL32p}. As can be seen, the predictions from SM1 and SM2 are nearly identical in both channels. The SUSY prediction is quite different from the SM predictions in both channels.

\subsubsection*{$\it\jp=5/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_L_52p.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_L_52p.eps}}
\caption{Same as Fig. \ref{fig:PL12p} but for $\Lambda_{b}\rightarrow\Lambda(1820)$.}\label{fig:PL52p}
\end{figure}

Fig. \ref{fig:PL52p} shows the predictions for LLPAs for decays to $\Ls(1820)$. It can be seen that the predictions from SM1 and SM2 are nearly identical in both channels. The SUSY prediction is different from those of the SM in both channels.

\subsubsection{Transverse Lepton Polarization Asymmetries}


\begin{table}
\caption{Integrated transverse lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\mu^{+}\mu^{-}$ in units of $10^{-2}$. The columns are labeled as in Table \ref{llpa1}.}
{\begin{tabular}{cccccc}
\hline State, $J^{P}$       & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2}  \\
& & & & &\small QCDSR $\,\,$\small PM   \\ \hline
$\Lambda(1115)\,1/2^{+}$   & a & $-0.07$ & $-0.07$ & $-0.04$ & $-0.07\,\,\,\,\,\,\,\,\,\,\,-0.07$ \\
                           & b & $-0.12$ & $-0.12$ & $-0.07$ & $-$  \\ \hline
$\Lambda(1600)\,1/2^{+}$   & a & $-0.05$ & $-0.05$ & $-0.03$ & $-$ \\
                           & b & $-0.06$ & $-0.06$ & $-0.04$ & $-$  \\ \hline
$\Lambda(1405)\,1/2^{-}$   & a & $-0.06$ & $-0.07$ & $-0.04$ & $-$  \\
                           & b & $-0.10$ & $-0.11$ & $-0.06$ & $-$  \\ \hline
$\Lambda(1520)\,3/2^{-}$   & a & $-0.04$ &  $-0.05$ & $-0.03$ & $-$  \\
                           & b & $-0.05$ & $-0.06$ & $-0.04$ & $-$  \\ \hline
$\Lambda(1890)\,3/2^{+}$   & a & $-0.03$ & $-0.03$ & $-0.02$ & $-$  \\
                           & b & $-0.02$ & $-0.03$ & $-0.02$ & $-$  \\ \hline
$\Lambda(1820)\,5/2^{+}$   & a & $-0.02$ &  $-0.02$ & $-0.01$ & $-$  \\
                           & b & $-0.01$ & $-0.02$ & $-0.01$ & $-$  \\ \hline
\end{tabular}\label{tlpa1}}
\end{table}

\begin{table}
\caption{Integrated transverse lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\tau^{+}\tau^{-}$ in units of $10^{-2}$. The columns are labeled as in Table \ref{llpa1}.}
{\begin{tabular}{ccccccc}
\hline State, $J^{P}$      & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2} \\
& & & & &\small QCDSR $\,\,$\small PM    \\ \hline
$\Lambda(1115)\,1/2^{+}$   & a & $-0.33$ & $-0.31$ & $-0.15$ & $-0.39\,\,\,\,\,\,\,\,\,\,\,-0.34$ \\
                           & b & $-0.57$ & $-0.54$ & $-0.27$ & $-$  \\ \hline
$\Lambda(1600)\,1/2^{+}$   & a & $-0.12$ & $-0.12$ & $-0.05$ & $-$ \\
                           & b & $-0.16$ & $-0.15$ & $-0.08$ & $-$  \\ \hline
$\Lambda(1405)\,1/2^{-}$   & a & $-0.22$ & $-0.24$ & $-0.11$ & $-$  \\
                           & b & $-0.38$ & $-0.41$ & $-0.20$ & $-$  \\ \hline
$\Lambda(1520)\,3/2^{-}$   & a & $-0.08$ &  $-0.10$ & $-0.04$ & $-$  \\
                           & b & $-0.11$ & $-0.14$ & $-0.07$ & $-$  \\ \hline
$\Lambda(1890)\,3/2^{+}$   & a & $-0.01$ & $-0.01$ & $-0.01$ & $-$  \\
                           & b & $\sim-\E{-3}$ & $-0.01$ & $-0.01$ & $-$  \\ \hline
$\Lambda(1820)\,5/2^{+}$   & a & $0.01$ &  $0.01$ & $0.01$ & $-$  \\
                           & b & $0.02$ & $0.02$ & $0.01$ & $-$  \\ \hline
\end{tabular}\label{tlpa2}}
\end{table}

The integrated TLPAs we obtain are shown in Tables \ref{tlpa1} and \ref{tlpa2}. The column labels have the same meaning as with LLPAs shown in Tables \ref{llpa1} and \ref{llpa2}. We also compare our results for decays to the ground state with those of Chen \etal \cite{chen2} (QCDSR and PM).

\subsubsection*{$\it\jp=1/2^+$}


\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_12p_mcn_hqet_lo.eps}\,\,\,\,\,\,
\includegraphics[width=3.0in]{tau_slpa_T_12p_mcn_hqet_lo.eps}}
\caption{$\P_T^-(\hat s)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$. The 
solid curves arise from the SM1 model, the dashed curves from SM2, the dot-dashed curves from HQET with the vector form factors from SCA model, the dash-dotted curves from HQET with the vector form factors from MCN model, and the thick solid curves from $\D_T^{(0)-}/\D_0^{(0)}$.}\label{fig:PTlo12p}
\end{figure}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_12p.eps}\,\,\,\,\,\,
\includegraphics[width=3.0in]{tau_slpa_T_12p.eps}}
\caption{$\P_T^-(\sh)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$ without and with long distance (LD) contributions from charmonium resonances. The solid and dashed curves represent SLPAs obtained from SCA and MCN form factors, respectively. The dash-dotted curves represent a SUSY extension to the SM.}\label{fig:PT12p}
\end{figure}



%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_12p1r.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_T_12p1r.eps}}
\caption{Same as Fig. \ref{fig:PT12p} but for $\Lambda_{b}\rightarrow\Lambda(1600)$.}\label{fig:PT12p1r}
\end{figure}



\subsubsection*{$\it\jp=1/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_12m_00.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_T_12m_00.eps}}
\caption{Same as Fig. \ref{fig:PT12p} but for $\Lambda_{b}\rightarrow\Lambda(1405)$.}\label{fig:PT12m}
\end{figure}



\subsubsection*{$\it\jp=3/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_32m.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_T_32m.eps}}
\caption{Same as Fig. \ref{fig:PT12p} but for $\Lambda_{b}\rightarrow\Lambda(1520)$.}\label{fig:PT32m}
\end{figure}



\subsubsection*{$\it\jp=3/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_32p_00.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_T_32p_00.eps}}
\caption{Same as Fig. \ref{fig:PT12p} but for $\Lambda_{b}\rightarrow\Lambda(1890)$.}\label{fig:PT32p}
\end{figure}



\subsubsection*{$\it\jp=5/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=3.0in]{mu_slpa_T_52p.eps}\,\,\,\,\,\, \includegraphics[width=3.0in]{tau_slpa_T_52p.eps}}
\caption{Same as Fig. \ref{fig:PT12p} but for $\Lambda_{b}\rightarrow\Lambda(1820)$.}\label{fig:PT52p}
\end{figure}



\subsubsection{Normal Lepton Polarization Asymmetries}

\begin{table}
\caption{Integrated normal lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\mu^{+}\mu^{-}$ in units of $10^{-2}$. The columns are labeled as in Table \ref{llpa1}.}
{\begin{tabular}{c|c|c|c|c|c}
\hline State, $J^{P}$       & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2} \\
& & & & &\small QCDSR $\,\,\,\,\,\,\,\,$\small PM  \\
& & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+\,\,\,\,\,\,\,\,\,\,\,-\,\,\,\,\,\,\,\,\,\,\,\,+$    \\ \hline
$\Lambda(1115)\,1/2^{+}$   & a & $5.1\,\,\,\,\,\,2.9$ & $5.1\,\,\,\,\,\,2.9$ & $5.5\,\,\,\,\,\,-0.02$ & $-\,\,\,\,\,\,-9.4\,\,\,\,\,\,\,\,\,\,\,-\,\,\,\,\,\,-12.6$ \\
                           & b & $5.0\,\,\,\,\,\,2.7$ & $4.9\,\,\,\,\,\,2.7$ & $5.3\,\,\,\,\,\,-0.13$ & $-$  \\ \hline
$\Lambda(1600)\,1/2^{+}$   & a & $4.9\,\,\,\,\,\,3.0$ & $4.7\,\,\,\,\,\,2.8$ & $5.1\,\,\,\,\,\,3.5$   & $-$ \\
                           & b & $4.7\,\,\,\,\,\,2.8$ & $4.6\,\,\,\,\,\,2.6$ & $4.9\,\,\,\,\,\,-0.09$ & $-$  \\ \hline
$\Lambda(1405)\,1/2^{-}$   & a & $4.9\,\,\,\,\,\,2.8$ & $4.9\,\,\,\,\,\,2.7$ & $5.3\,\,\,\,\,\,-0.17$ & $-$  \\
                           & b & $4.8\,\,\,\,\,\,2.6$ & $4.8\,\,\,\,\,\,2.5$ & $5.1\,\,\,\,\,\,-0.28$ & $-$  \\ \hline
$\Lambda(1520)\,3/2^{-}$   & a & $4.6\,\,\,\,\,\,2.7$ & $4.6\,\,\,\,\,\,2.8$ & $5.0\,\,\,\,\,\,-0.02$ & $-$  \\
                           & b & $4.5\,\,\,\,\,\,2.5$ & $4.6\,\,\,\,\,\,2.6$ & $4.8\,\,\,\,\,\,-0.13$ & $-$  \\ \hline
$\Lambda(1890)\,3/2^{+}$   & a & $4.4\,\,\,\,\,\,2.7$ & $4.3\,\,\,\,\,\,2.5$ & $4.6\,\,\,\,\,\,-0.13$ & $-$  \\
                           & b & $4.3\,\,\,\,\,\,2.5$ & $4.3\,\,\,\,\,\,2.3$ & $4.4\,\,\,\,\,\,-0.25$ & $-$  \\ \hline
$\Lambda(1820)\,5/2^{+}$   & a & $4.3\,\,\,\,\,\,2.6$ & $4.3\,\,\,\,\,\,2.7$ & $4.6\,\,\,\,\,\,-0.09$ & $-$  \\
                           & b & $4.2\,\,\,\,\,\,2.4$ & $4.2\,\,\,\,\,\,2.5$ & $4.4\,\,\,\,\,\,-0.20$ & $-$  \\ \hline
\end{tabular}\label{nlpa1}}
\end{table}

\begin{table}
\caption{Integrated normal lepton polarization asymmetry for $\Lambda_b\rightarrow \Lambda^{(*)}\tau^{+}\tau^{-}$ in units of $10^{-2}$. The columns are labeled as in Table \ref{llpa1}.}
{\begin{tabular}{c|c|c|c|c|c}
\hline State, $J^{P}$      & LD & SM1 & SM2 & SUSY & Chen {\it et al.} \cite{chen2}  \\
& & & & &\small QCDSR $\,\,\,\,\,\,\,\,$\small PM  \\
& & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+$ & $-\,\,\,\,\,\,\,\,\,\,\,\,+\,\,\,\,\,\,\,\,\,\,\,-\,\,\,\,\,\,\,\,\,\,\,\,+$    \\ \hline
$\Lambda(1115)\,1/2^{+}$   & a & $13.6\,\,\,\,\,\,4.9$ & $13.3\,\,\,\,\,\,4.9$ & $13.4\,\,\,\,\,\,-0.89$ & $-\,\,\,\,\,\,-10.0\,\,\,\,\,\,\,\,\,\,\,-\,\,\,\,\,\,-9.2$ \\
                           & b & $12.9\,\,\,\,\,\,4.1$ & $12.7\,\,\,\,\,\,4.1$ & $13.1\,\,\,\,\,\,-1.1$ & $-$  \\ \hline
$\Lambda(1600)\,1/2^{+}$   & a & $7.5\,\,\,\,\,\,3.3$ & $7.2\,\,\,\,\,\,3.0$ & $7.1\,\,\,\,\,\,-0.29$ & $-$ \\
                           & b & $6.9\,\,\,\,\,\,2.5$ & $6.7\,\,\,\,\,\,2.3$ & $6.8\,\,\,\,\,\,-0.52$ & $-$  \\ \hline
$\Lambda(1405)\,1/2^{-}$   & a & $10.7\,\,\,\,\,\,4.2$ & $10.9\,\,\,\,\,\,3.7$ & $11.0\,\,\,\,\,\,-0.97$ & $-$  \\
                           & b & $10.1\,\,\,\,\,\,3.3$ & $10.3\,\,\,\,\,\,2.9$ & $10.6\,\,\,\,\,\,-1.2$ & $-$  \\ \hline
$\Lambda(1520)\,3/2^{-}$   & a & $6.4\,\,\,\,\,\,3.9$ &  $6.9\,\,\,\,\,\,3.5$ & $6.6\,\,\,\,\,\,-0.06$ & $-$  \\
                           & b & $5.9\,\,\,\,\,\,3.2$ & $6.4\,\,\,\,\,\,2.8$ & $6.3\,\,\,\,\,\,-0.28$ & $-$  \\ \hline
$\Lambda(1890)\,3/2^{+}$   & a & $1.7\,\,\,\,\,\,1.4$ & $2.1\,\,\,\,\,\,1.2$ & $2.0\,\,\,\,\,\,0.10$ & $-$  \\
                           & b & $1.4\,\,\,\,\,\,0.94$ & $1.9\,\,\,\,\,\,0.68$ & $1.7\,\,\,\,\,\,-0.13$ & $-$  \\ \hline
$\Lambda(1820)\,5/2^{+}$   & a & $1.9\,\,\,\,\,\,2.9$ &  $1.9\,\,\,\,\,\,2.8$ & $1.7\,\,\,\,\,\,0.85$ & $-$  \\
                           & b & $1.6\,\,\,\,\,\,2.3$ & $1.6\,\,\,\,\,\,2.2$ & $1.5\,\,\,\,\,\,0.66$ & $-$  \\ \hline
\end{tabular}\label{nlpa2}}
\end{table}

The integrated NLPAs we obtain are shown in Tables \ref{nlpa1} and \ref{nlpa2}. The column labels have the same meaning as with LLPAs shown in Tables \ref{llpa1} and \ref{llpa2}. We also compare our results for decays to the ground state with those of Chen \etal \cite{chen2} (QCDSR and PM).

\subsubsection*{$\it\jp=1/2^+$}


%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_12p_mcn_hqet_lo.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_12p_mcn_hqet_lo.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_12p_mcn_hqet_lo.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_12p_mcn_hqet_lo.eps}}
\caption{$\P_N^-(\sh)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$ without and with long distance (LD) contributions from charmonium resonances. $\P_N^+(\sh)$ for the $\mu$ and $\tau$ channels are also shown in (c) and (d), respectively. The solid curves arise from the SM1 model, the dashed curves from SM2, the dot-dashed curves from HQET with the vector form factors from SCA model, the dash-dotted curves from HQET with the vector form factors from MCN model, and the thick solid curves from $\D_N^{(0)\pm}/\D_0^{(0)}$.}\label{fig:PNlo12p}
\end{figure}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_12p.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_12p.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_12p.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_12p.eps}}
\caption{$\P_N^-(\sh)$ for (a) $\Lambda_{b}\rightarrow\Lambda(1115)\mu^{+}\mu^{-}$ and (b) $\Lambda_{b}\rightarrow\Lambda(1115)\tau^{+}\tau^{-}$ without and with long distance (LD) contributions from charmonium resonances. $\P_N^+(\sh)$ for the $\mu$ and $\tau$ channels are also shown in (c) and (d), respectively. The solid and dashed curves represent SLPAs obtained from SCA and MCN form factors, respectively. The dash-dotted curves represent a SUSY extension to the SM.}\label{fig:PN12p}
\end{figure}



%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_12p1r.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_12p1r.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_12p1r.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_12p1r.eps}}
\caption{Same as Fig. \ref{fig:PN12p} but for $\Lambda_{b}\rightarrow\Lambda(1600)$.}\label{fig:PN12p1r}
\end{figure}



\subsubsection*{$\it\jp=1/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_12m_00.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_12m_00.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_12m_00.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_12m_00.eps}}
\caption{Same as Fig. \ref{fig:PN12p} but for $\Lambda_{b}\rightarrow\Lambda(1405)$.}\label{fig:PN12m}
\end{figure}



\subsubsection*{$\it\jp=3/2^-$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_32m.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_32m.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_32m.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_32m.eps}}
\caption{Same as Fig. \ref{fig:PN12p} but for $\Lambda_{b}\rightarrow\Lambda(1520)$.}\label{fig:PN32m}
\end{figure}



\subsubsection*{$\it\jp=3/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_32p_00.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_32p_00.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_32p_00.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_32p_00.eps}}
\caption{Same as Fig. \ref{fig:PN12p} but for $\Lambda_{b}\rightarrow\Lambda(1890)$.}\label{fig:PN32p}
\end{figure}



\subsubsection*{$\it\jp=5/2^+$}

%\vskip 0.5in
\begin{figure}
\centerline{\includegraphics[width=2.5in]{mu_slpa_N_52p.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N_52p.eps}}\vskip25pt
\centerline{\includegraphics[width=2.5in]{mu_slpa_N2_52p.eps}\hskip30pt \includegraphics[width=2.5in]{tau_slpa_N2_52p.eps}}
\caption{Same as Fig. \ref{fig:PN12p} but for $\Lambda_{b}\rightarrow\Lambda(1820)$.}\label{fig:PN52p}
\end{figure}



==> sca_ff.tex <==
\section{Analytic Form Factors\label{sec:aff}}

Here we present the vector, axial-vector, and tensor form factors obtained from single-component quark model wave functions in the oscillator basis.
These form factors were extracted using a nonrelativistic reduction of the quark current. The resulting form factors have the form of a polynomial in
the daughter baryon momentum $\pls$ times a Gaussian. The polynomials in the form factors presented here are truncated at zeroth order in $\pls$.

\subsection{${1/2}^{+}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ \frac{m_q \alpha _{\lambda }^2}{m_b \alpha _{\lambda \lambda
   '}^2}+\frac{m_q \alpha _{\lambda '}^2}{m_s \alpha _{\lambda \lambda
   '}^2}+1 \bigg] \\
F_2&=&I_H\bigg[ \frac{\alpha _{\lambda }^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha
   _{\lambda \lambda '}^2}-\frac{m_q \alpha _{\lambda '}^2}{m_s \alpha
   _{\lambda \lambda '}^2} \bigg] \\
F_3&=&I_H\bigg[ -\frac{m_q \alpha _{\lambda }^2}{m_b \alpha _{\lambda \lambda '}^2} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ 1-\frac{\alpha _{\lambda }^2 \alpha _{\lambda '}^2}{12 m_b m_s \alpha
   _{\lambda \lambda '}^2} \bigg] \\
G_2&=&I_H\bigg[ -\frac{m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}-\frac{\alpha _{\lambda }^2 \alpha _{\lambda
   '}^2}{12 m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{m_q \alpha
   _{\lambda '}^2}{m_s \alpha _{\lambda \lambda '}^2} \bigg] \\
G_3&=&I_H\bigg[ \frac{m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{m_q \alpha _{\lambda }^2}{m_b \alpha
   _{\lambda \lambda '}^2} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ \frac{\alpha _{\lambda }^2 \alpha _{\lambda '}^2}{12 m_b m_s \alpha
   _{\lambda \lambda '}^2}+1 \bigg] \\
H_2&=&I_H\bigg[ \frac{m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}-\frac{\alpha _{\lambda }^2 \alpha _{\lambda
   '}^2}{12 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{m_q \alpha
   _{\lambda '}^2}{m_s \alpha _{\lambda \lambda '}^2} \bigg] \\
H_3&=&I_H\bigg[ -\frac{m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}-\frac{m_q \alpha _{\lambda }^2}{m_b \alpha
   _{\lambda \lambda '}^2} \bigg] \\
H_4&=&I_H\bigg[ -\frac{m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4} \bigg]
\end{eqnarray*}

$$
I_{H}=\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{3/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$

\subsection{${1/2_{1}}^{+}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ \frac{m_q \alpha _{\lambda }^2 \left(3 \alpha _{\lambda }^2-7 \alpha
   _{\lambda '}^2\right)}{6 m_b \alpha _{\lambda \lambda '}^4}+\frac{m_q
   \alpha _{\lambda '}^2 \left(7 \alpha _{\lambda }^2-3 \alpha _{\lambda
   '}^2\right)}{6 m_s \alpha _{\lambda \lambda '}^4}+\frac{\alpha
   _{\lambda }^2-\alpha _{\lambda '}^2}{2 \alpha _{\lambda \lambda '}^2} \bigg] \\
F_2&=&I_H\bigg[ \frac{\alpha _{\lambda }^2 \alpha _{\lambda '}^2 \left(7 \alpha _{\lambda
   }^2-3 \alpha _{\lambda '}^2\right)}{24 m_b m_s \alpha _{\lambda \lambda
   '}^4}-\frac{m_q \alpha _{\lambda '}^2 \left(7 \alpha _{\lambda }^2-3
   \alpha _{\lambda '}^2\right)}{6 m_s \alpha _{\lambda \lambda '}^4} \bigg] \\
F_3&=&I_H\bigg[ -\frac{m_q \alpha _{\lambda }^2 \left(3 \alpha _{\lambda }^2-7 \alpha
   _{\lambda '}^2\right)}{6 m_b \alpha _{\lambda \lambda '}^4} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ \frac{\alpha _{\lambda }^2-\alpha _{\lambda '}^2}{2 \alpha _{\lambda
   \lambda '}^2}-\frac{\alpha _{\lambda }^2 \alpha _{\lambda '}^2 \left(7
   \alpha _{\lambda }^2-3 \alpha _{\lambda '}^2\right)}{72 m_b m_s \alpha
   _{\lambda \lambda '}^4} \bigg] \\
G_2&=&I_H\bigg[ -\frac{7 m_q^2 \alpha _{\lambda }^2 \left(\alpha _{\lambda }^2-\alpha
   _{\lambda '}^2\right) \alpha _{\lambda '}^2}{6 m_b m_s \alpha _{\lambda
   \lambda '}^6}-\frac{\alpha _{\lambda }^2 \left(7 \alpha _{\lambda }^2-3
   \alpha _{\lambda '}^2\right) \alpha _{\lambda '}^2}{72 m_b m_s \alpha
   _{\lambda \lambda '}^4}-\frac{m_q \left(7 \alpha _{\lambda }^2-3 \alpha
   _{\lambda '}^2\right) \alpha _{\lambda '}^2}{6 m_s \alpha _{\lambda
   \lambda '}^4} \bigg] \\
G_3&=&I_H\bigg[ \frac{7 m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2 \left(\alpha
   _{\lambda }^2-\alpha _{\lambda '}^2\right)}{6 m_b m_s \alpha _{\lambda
   \lambda '}^6}+\frac{m_q \alpha _{\lambda }^2 \left(3 \alpha _{\lambda
   }^2-7 \alpha _{\lambda '}^2\right)}{6 m_b \alpha _{\lambda \lambda
   '}^4} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ \frac{\alpha _{\lambda }^2 \left(7 \alpha _{\lambda }^2-3 \alpha _{\lambda
   '}^2\right) \alpha _{\lambda '}^2}{72 m_b m_s \alpha _{\lambda \lambda
   '}^4}+\frac{\alpha _{\lambda }^2-\alpha _{\lambda '}^2}{2 \alpha
   _{\lambda \lambda '}^2} \bigg] \\
H_2&=&I_H\bigg[ \frac{7 m_q^2 \alpha _{\lambda }^2 \left(\alpha _{\lambda }^2-\alpha
   _{\lambda '}^2\right) \alpha _{\lambda '}^2}{6 m_b m_s \alpha _{\lambda
   \lambda '}^6}-\frac{\alpha _{\lambda }^2 \left(7 \alpha _{\lambda }^2-3
   \alpha _{\lambda '}^2\right) \alpha _{\lambda '}^2}{72 m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{m_q \left(7 \alpha _{\lambda }^2-3 \alpha
   _{\lambda '}^2\right) \alpha _{\lambda '}^2}{6 m_s \alpha _{\lambda
   \lambda '}^4} \bigg] \\
H_3&=&I_H\bigg[ -\frac{7 m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2 \left(\alpha
   _{\lambda }^2-\alpha _{\lambda '}^2\right)}{6 m_b m_s \alpha _{\lambda
   \lambda '}^6}-\frac{m_q \alpha _{\lambda }^2 \left(3 \alpha _{\lambda
   }^2-7 \alpha _{\lambda '}^2\right)}{6 m_b \alpha _{\lambda \lambda
   '}^4} \bigg] \\
H_4&=&I_H\bigg[ -\frac{7 m_q^2 \alpha _{\lambda }^2 \alpha _{\lambda '}^2 \left(\alpha
   _{\lambda }^2-\alpha _{\lambda '}^2\right)}{6 m_b m_s \alpha _{\lambda
   \lambda '}^6} \bigg]
\end{eqnarray*}

$$
I_{H}=\sqrt{\frac{3}{2}}\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{3/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$

\subsection{${1/2}^{-}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ \frac{\alpha _{\lambda }}{2 m_s}-\frac{\alpha _{\lambda }}{6 m_b} \bigg] \\
F_2&=&I_H\bigg[ \frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda }^2-2 \alpha _{\lambda '}^2\right)}{6
   m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{2 m_q^2 \alpha _{\lambda }}{m_b \alpha
   _{\lambda \lambda '}^2}-\frac{2 m_q}{\alpha _{\lambda }}+\frac{\alpha _{\lambda }}{2
   m_s} \bigg] \\
F_3&=&I_H\bigg[ \frac{2 m_q^2 \alpha _{\lambda }}{m_b \alpha _{\lambda \lambda '}^2} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ \frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda }^2-2 \alpha _{\lambda '}^2\right)}{6
   m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{\alpha _{\lambda }}{6 m_b}+\frac{2
   m_q}{\alpha _{\lambda }} \bigg] \\
G_2&=&I_H\bigg[ \frac{\alpha _{\lambda }}{3 m_b}-\frac{2 m_q}{\alpha _{\lambda }}+\frac{\alpha _{\lambda
   }}{2 m_s} \bigg] \\
G_3&=&I_H\bigg[ \frac{\alpha _{\lambda }}{3 m_b}-\frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda
   }^2-2 \alpha _{\lambda '}^2\right)}{6 m_b m_s \alpha _{\lambda \lambda '}^2} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ -\frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda }^2-2 \alpha _{\lambda
   '}^2\right)}{6 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{\alpha _{\lambda }}{2
   m_b}-\frac{2 m_q}{\alpha _{\lambda }} \bigg] \\
H_2&=&I_H\bigg[ \frac{\alpha _{\lambda }}{3 m_b}-\frac{2 m_q}{\alpha _{\lambda }}+\frac{\alpha _{\lambda
   }}{2 m_s} \bigg] \\
H_3&=&I_H\bigg[ \frac{\alpha _{\lambda }}{3 m_b}-\frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda
   }^2-2 \alpha _{\lambda '}^2\right)}{6 m_b m_s \alpha _{\lambda \lambda '}^2} \bigg] \\
H_4&=&I_H\bigg[ \frac{m_q \alpha _{\lambda } \left(3 \alpha _{\lambda }^2-2 \alpha _{\lambda '}^2\right)}{6
   m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{2 m_q^2 \alpha _{\lambda }}{m_b \alpha
   _{\lambda \lambda '}^2}-\frac{\alpha _{\lambda }}{3 m_b} \bigg]
\end{eqnarray*}

$$
I_{H}=\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{5/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$

\subsection{${3/2}^{-}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ -\frac{3 m_q^2 \alpha _{\lambda }}{m_b \alpha _{\lambda \lambda
   '}^2}-\frac{3 m_q^2 \alpha _{\lambda '}^2}{m_s \alpha _{\lambda }
   \alpha _{\lambda \lambda '}^2}-\frac{3 m_q}{\alpha _{\lambda }} \bigg] \\
F_2&=&I_H\bigg[ \frac{3 m_q^2 \alpha _{\lambda '}^2}{m_s \alpha _{\lambda } \alpha
   _{\lambda \lambda '}^2}-\frac{5 m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{4 m_b m_s \alpha _{\lambda \lambda '}^2} \bigg] \\
F_3&=&I_H\bigg[ \frac{3 m_q^2 \alpha _{\lambda }}{m_b \alpha _{\lambda \lambda
   '}^2}+\frac{\alpha _{\lambda }}{2 m_b} \bigg] \\
F_4&=&I_H\bigg[ -\frac{\alpha _{\lambda }}{m_b} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ \frac{3 m_q \alpha _{\lambda } \alpha _{\lambda '}^2}{4 m_b m_s \alpha
   _{\lambda \lambda '}^2}+\frac{\alpha _{\lambda }}{2 m_b}-\frac{3
   m_q}{\alpha _{\lambda }} \bigg] \\
G_2&=&I_H\bigg[ \frac{3 m_q^3 \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{4 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{3 m_q^2 \alpha
   _{\lambda '}^2}{m_s \alpha _{\lambda } \alpha _{\lambda \lambda '}^2} \bigg] \\
G_3&=&I_H\bigg[ -\frac{3 m_q^3 \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}-\frac{m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{2 m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{3 m_q^2 \alpha
   _{\lambda }}{m_b \alpha _{\lambda \lambda '}^2}-\frac{\alpha _{\lambda
   }}{2 m_b} \bigg] \\
G_4&=&I_H\bigg[ \frac{m_q \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^2}+\frac{\alpha _{\lambda }}{m_b} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ -\frac{7 m_q \alpha _{\lambda } \alpha _{\lambda '}^2}{4 m_b m_s \alpha
   _{\lambda \lambda '}^2}-\frac{3 \alpha _{\lambda }}{2 m_b}-\frac{3
   m_q}{\alpha _{\lambda }} \bigg] \\
H_2&=&I_H\bigg[ -\frac{3 m_q^3 \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{9 m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{4 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{2 \alpha _{\lambda
   }}{m_b}-\frac{3 m_q^2 \alpha _{\lambda '}^2}{m_s \alpha _{\lambda }
   \alpha _{\lambda \lambda '}^2} \bigg] \\
H_3&=&I_H\bigg[ \frac{3 m_q^3 \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{2 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{3 m_q^2 \alpha
   _{\lambda }}{m_b \alpha _{\lambda \lambda '}^2}+\frac{\alpha _{\lambda
   }}{2 m_b} \bigg] \\
H_4&=&I_H\bigg[ \frac{3 m_q^3 \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^4}+\frac{m_q \alpha _{\lambda } \alpha _{\lambda
   '}^2}{2 m_b m_s \alpha _{\lambda \lambda '}^2} \bigg] \\
H_5&=&I_H\bigg[ -\frac{m_q \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^2}-\frac{\alpha _{\lambda }}{m_b} \bigg] \\
H_6&=&I_H\bigg[ \frac{m_q \alpha _{\lambda } \alpha _{\lambda '}^2}{m_b m_s \alpha
   _{\lambda \lambda '}^2} \bigg]
\end{eqnarray*}

$$
I_{H}=-\frac{1}{\sqrt{3}}\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{5/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$

\subsection{${3/2}^{+}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ \frac{3 m_q}{2 m_b}-\frac{5 m_q}{2 m_s} \bigg] \\
F_2&=&I_H\bigg[ -\frac{m_q^2 \left(5 \alpha _{\lambda }^2-2 \alpha _{\lambda
   '}^2\right)}{2 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{6
   m_q^3}{m_b \alpha _{\lambda \lambda '}^2}-\frac{5 m_q}{2 m_s}+\frac{6
   m_q^2}{\alpha _{\lambda }^2} \bigg] \\
F_3&=&I_H\bigg[ -\frac{6 m_q^3}{m_b \alpha _{\lambda \lambda '}^2}-\frac{m_q}{m_b} \bigg] \\
F_4&=&I_H\bigg[ \frac{2 m_q}{m_b} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ -\frac{m_q^2 \left(5 \alpha _{\lambda }^2-2 \alpha _{\lambda
   '}^2\right)}{2 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{m_q}{2
   m_b}-\frac{6 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
G_2&=&I_H\bigg[ -\frac{2 m_q}{m_b}+\frac{5 \alpha _{\lambda }^2}{12 m_b m_s}-\frac{5
   m_q}{2 m_s}+\frac{6 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
G_3&=&I_H\bigg[ \frac{7 m_q^2 \alpha _{\lambda }^2}{2 m_b m_s \alpha _{\lambda \lambda
   '}^2}-\frac{2 m_q^2}{m_b m_s}-\frac{m_q}{m_b}+\frac{5 \alpha _{\lambda
   }^2}{12 m_b m_s} \bigg] \\
G_4&=&I_H\bigg[ -\frac{5 \alpha _{\lambda }^2}{6 m_b m_s} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ \frac{m_q^2 \left(5 \alpha _{\lambda }^2-2 \alpha _{\lambda '}^2\right)}{2
   m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{3 m_q}{2 m_b}+\frac{6
   m_q^2}{\alpha _{\lambda }^2} \bigg] \\
H_2&=&I_H\bigg[ -\frac{2 m_q}{m_b}+\frac{5 \alpha _{\lambda }^2}{12 m_b m_s}-\frac{5
   m_q}{2 m_s}+\frac{6 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
H_3&=&I_H\bigg[ \frac{m_q^2 \left(5 \alpha _{\lambda }^2-2 \alpha _{\lambda '}^2\right)}{2
   m_b m_s \alpha _{\lambda \lambda '}^2}-\frac{m_q}{m_b}+\frac{5 \alpha
   _{\lambda }^2}{12 m_b m_s} \bigg] \\
H_4&=&I_H\bigg[ -\frac{m_q^2 \left(5 \alpha _{\lambda }^2-2 \alpha _{\lambda
   '}^2\right)}{2 m_b m_s \alpha _{\lambda \lambda '}^2}+\frac{6
   m_q^3}{m_b \alpha _{\lambda \lambda '}^2}+\frac{2 m_q}{m_b}-\frac{5
   \alpha _{\lambda }^2}{12 m_b m_s} \bigg] \\
H_5&=&I_H\bigg[ -\frac{5 \alpha _{\lambda }^2}{6 m_b m_s} \bigg] \\
H_6&=&I_H\bigg[ \frac{2 m_q}{m_b}-\frac{5 \alpha _{\lambda }^2}{6 m_b m_s} \bigg]
\end{eqnarray*}

$$
I_{H}=\frac{1}{\sqrt{5}}\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{7/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$

\subsection{${5/2}^{+}$}

\begin{eqnarray*}
F_1&=&I_H\bigg[ \frac{3 m_q^3}{m_b \alpha _{\lambda \lambda '}^2}+\frac{3 m_q^3 \alpha
   _{\lambda '}^2}{m_s \alpha _{\lambda }^2 \alpha _{\lambda \lambda
   '}^2}+\frac{3 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
F_2&=&I_H\bigg[ \frac{7 m_q^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha _{\lambda \lambda
   '}^2}-\frac{3 m_q^3 \alpha _{\lambda '}^2}{m_s \alpha _{\lambda }^2
   \alpha _{\lambda \lambda '}^2} \bigg] \\
F_3&=&I_H\bigg[ -\frac{3 m_q^3}{m_b \alpha _{\lambda \lambda '}^2}-\frac{m_q}{m_b} \bigg] \\
F_4&=&I_H\bigg[ \frac{2 m_q}{m_b} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
G_1&=&I_H\bigg[ -\frac{5 m_q^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha _{\lambda \lambda
   '}^2}-\frac{m_q}{m_b}+\frac{3 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
G_2&=&I_H\bigg[ -\frac{3 m_q^4 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^4}-\frac{m_q^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha _{\lambda
   \lambda '}^2}-\frac{3 m_q^3 \alpha _{\lambda '}^2}{m_s \alpha _{\lambda
   }^2 \alpha _{\lambda \lambda '}^2} \bigg] \\
G_3&=&I_H\bigg[ \frac{3 m_q^4 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^4}+\frac{m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda
   \lambda '}^2}+\frac{3 m_q^3}{m_b \alpha _{\lambda \lambda
   '}^2}+\frac{m_q}{m_b} \bigg] \\
G_4&=&I_H\bigg[ -\frac{2 m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^2}-\frac{2 m_q}{m_b} \bigg]
\end{eqnarray*}


\begin{eqnarray*}
H_1&=&I_H\bigg[ \frac{13 m_q^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha _{\lambda \lambda
   '}^2}+\frac{3 m_q}{m_b}+\frac{3 m_q^2}{\alpha _{\lambda }^2} \bigg] \\
H_2&=&I_H\bigg[ \frac{3 m_q^4 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^4}-\frac{17 m_q^2 \alpha _{\lambda '}^2}{4 m_b m_s \alpha _{\lambda
   \lambda '}^2}-\frac{4 m_q}{m_b}+\frac{3 m_q^3 \alpha _{\lambda
   '}^2}{m_s \alpha _{\lambda }^2 \alpha _{\lambda \lambda '}^2} \bigg] \\
H_3&=&I_H\bigg[ -\frac{3 m_q^4 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^4}-\frac{m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda
   \lambda '}^2}-\frac{3 m_q^3}{m_b \alpha _{\lambda \lambda
   '}^2}-\frac{m_q}{m_b} \bigg] \\
H_4&=&I_H\bigg[ -\frac{3 m_q^4 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^4}-\frac{m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda
   \lambda '}^2} \bigg] \\
H_5&=&I_H\bigg[ \frac{2 m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^2}+\frac{2 m_q}{m_b} \bigg] \\
H_6&=&I_H\bigg[ -\frac{2 m_q^2 \alpha _{\lambda '}^2}{m_b m_s \alpha _{\lambda \lambda
   '}^2} \bigg]
\end{eqnarray*}

$$
I_{H}=\frac{1}{\sqrt{2}}\bigg(\frac{\alpha_{\lambda}\alpha_{\lambda'}}{\alpha_{\lambda\lambda'}^2}
\bigg)^{7/2}\exp\bigg(-\frac{3m_q^2}{2\widetilde{m}_{\Lambda}^2}
\frac{p_{\Lambda}^2}{\alpha_{\lambda\lambda'}^2}\bigg)
$$


